Hitting forbidden subgraphs in graphs of bounded treewidth

We study the complexity of a generic hitting problem H-Subgraph Hitting, where given a fixed pattern graph $H$ and an input graph $G$, the task is to find a set $X \subseteq V(G)$ of minimum size that hits all subgraphs of $G$ isomorphic to $H$. In the colorful variant of the problem, each vertex of $G$ is precolored with some color from $V(H)$ and we require to hit only $H$-subgraphs with matching colors. Standard techniques shows that for every fixed $H$, the problem is fixed-parameter tractable parameterized by the treewidth of $G$; however, it is not clear how exactly the running time should depend on treewidth. For the colorful variant, we demonstrate matching upper and lower bounds showing that the dependence of the running time on treewidth of $G$ is tightly governed by $\mu(H)$, the maximum size of a minimal vertex separator in $H$. That is, we show for every fixed $H$ that, on a graph of treewidth $t$, the colorful problem can be solved in time $2^{\mathcal{O}(t^{\mu(H)})}\cdot|V(G)|$, but cannot be solved in time $2^{o(t^{\mu(H)})}\cdot |V(G)|^{O(1)}$, assuming the Exponential Time Hypothesis (ETH). Furthermore, we give some preliminary results showing that, in the absence of colors, the parameterized complexity landscape of H-Subgraph Hitting is much richer.

==> boring.tex <==
\section{Boring proofs}\label{sec:boring}

\begin{proof}[of Lemma~\ref{lem:preprocess}]
First, preprocess $\Phi$ as follows:
\begin{enumerate}
\item Simplify all clauses that contain repeated variables: delete all clauses
that contain both a variable and its negation, and remove duplicate literals
from the remaining clauses.
\item As long as there exists a variable $x$ that appears only positively or only
negatively, fix the evaluation of $x$ that satisfies all clauses containing $x$
and simplify the formula.
\item As long as there exists a clause $C$ with only one literal, fix the evaluation
of this literal that satisfies $C$ and simplify the formula.
\item If some clause becomes empty in the process, return a dummy unsatisfiable clean formula.
\end{enumerate}
Observe that after this preprocessing, the size of $\Phi$ only shrinks,
while each variable appears at least twice.

Second, replace every variable $x$ with a cycle of implications
$x_1 \Rightarrow x_2 \Rightarrow \ldots \Rightarrow x_{s(x)} \Rightarrow x_1$, where
$s(x)$ is the number of appearances of $x$ in $\Phi$.
More formally, for every variable $x$:
\begin{enumerate}
\item introduce $s(x)$ new variables $x_1, x_2, \ldots, x_{s(x)}$, and replace
each occurence of $x$ in $\Phi$ with a distinct variable $x_i$; and
\item introduce $s(x)$ new clauses $x_i \Rightarrow x_{i+1}$ (i.e., $\neg x_i \vee x_{i+1}$)
  for $i=1,2,\ldots,s(x)$, where $x_{s(x)+1} = x_1$.
\end{enumerate}
Observe that, after this replacement, each variable $x_i$ appears exactly three times in
the formula $\Phi$: positively in the implication $x_{i-1} \Rightarrow x_i$,
negatively in the implication $x_i \Rightarrow x_{i+1}$ (with the convention $x_0 = x_{s(x)}$
and $x_{s(x)+1} = x_1$), and the third time in one former place of the variable $x$.
Moreover, as after the first step each variable appears at least twice in $\Phi$,
for every former
variable $x$ we have $s(x) \geq 2$ and no new clause contains twice the same variable.
Finally, note that the second step increases the size of the formula by a constant factor.
The lemma follows.
\maybeqed\end{proof}

